Parameter-Efficient and Memory-Efficient Tuning for Vision Transformer: A Disentangled Approach

Recent works on parameter-efficient transfer learning (PETL) show the potential to adapt a pre-trained Vision Transformer to downstream recognition tasks with only a few learnable parameters. However, since they usually insert new structures into the pre-trained model, entire intermediate features of that model are changed and thus need to be stored to be involved in back-propagation, resulting in memory-heavy training. We solve this problem from a novel disentangled perspective, i.e., dividing PETL into two aspects: task-specific learning and pre-trained knowledge utilization. Specifically, we synthesize the task-specific query with a learnable and lightweight module, which is independent of the pre-trained model. The synthesized query equipped with task-specific knowledge serves to extract the useful features for downstream tasks from the intermediate representations of the pre-trained model in a query-only manner. Built upon these features, a customized classification head is proposed to make the prediction for the input sample. lightweight architecture and avoids the use of heavy intermediate features for running gradient descent, it demonstrates limited memory usage in training. Extensive experiments manifest that our method achieves state-of-the-art performance under memory constraints, showcasing its applicability in real-world situations.

==> sec/2_related.tex <==
\section{Related Work}
\noindent\textbf{Parameter-Efficient transfer learning (PETL).}
PETL has attracted much attention and has been widely explored in recent
works \cite{hu2021lora,tu2023visual,chen2022adaptformer, lian2022scaling,jia2022visual}. 
PETL reduces computational cost of transferring knowledge from large pretrained models to new tasks, by avoiding updates of the entire parameters. 
BitFit \cite{zaken2021bitfit} only finetunes the bias in transfer learning and shows comparable performance to full tuning. Adapter \cite{houlsby2019parameter} adopts bottleneck structures after the projection following multiheaded attention and after the two feed-forward layers. 
LoRA \cite{hu2021lora} observes that the learned over-parametrized models reside on a low-rank dimension and further injects trainable rank decomposition parameters into each layer of transformer. 
VPT \cite{jia2022visual} introduces PETL to vision transformer and inserts learnable prompts into the token space. 
AdaptFormer \cite{chen2022adaptformer} adds parallel lightweight module to the feed-forward network, while SSF \cite{lian2022scaling} performs scaling and shifting for domain adaptation. FactT \cite{jie2023fact} applys tensorization-decomposition framework for parameters-saving and Binary Adapter \cite{jie2023revisiting} shows excellent performance with a computational-efficient quantization module. 

\noindent\textbf{Intermediate features mining for Memory-Efficient transfer learning}
Although PETL have shown promising performance in transfer learning while saving most trainable parameters, they still suffer from issues of high memory consumption. The full back-propagation throughout the entire backbone prevent traditional PETL methods from applying in memory-constraint situations. Recently, some approaches have been proposed and is capable to address such issues by leveraging the power of intermediate representations of a pretrained model \cite{sung2022lst,tu2023visual,evci2022head2toe}. 
LST \cite{sung2022lst} proposes a lightweight trainable structures in the sideway called ladders for the purpose of memory-saving during training. 
Head2Toe \cite{evci2022head2toe} selects features from all layers of the source model to feed into a classification head for the target domain. VQT \cite{tu2023visual} inserts trainable token in the query space to apply information mining of the pretrained model. Due to the information redundancy in the intermediate representations, both Head2Toe and VQT further applys group lasso \cite{yuan2006model} for feature selection. 

In contrast to previous methods, we provide an insightful analysis that the entangled combination of task-specific
learning and pre-trained knowledge utilization result in high memory consumption of traditional PETL method. Therefore, we propose SynQT, designed to disentangle PETL into two distinct modules, with the aim of capturing task-specific knowledge and implementing intermediate information mining, respectively. Such disentangled paradigm enjoys memory efficiency in transfer learning compared with traditional PETL methods. 


==> sec/3_method.tex <==
% \section{Method}
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.95\textwidth,page=3]{pdf/framework.pdf}
%     \caption{Overall architecture of SynQT.}
%     \label{framework}
% \end{figure*}
\subsection{Overall Architecture}
As can be seen from Figure \ref{framework}, SynQT can be mainly divided into two parts: Query Synthesis Module (QSM) and Knowledge Extraction Module (KEM).
Query Synthesis Module is a light-weight transformer block, which is used to capture task-specific knowledge, bridging the gap between the downstream tasks and knowledge from the pretrained model.
Knowledge Extraction Module uses the results generated by QSM as queries, and the intermediate features in the pretrained ViT as keys and values. It reuses the original ViT model's parameter weights to extract features that are beneficial to downstream classification tasks.
The rich hierarchical features extracted by the Knowledge Extraction are input into a classification head, as shown in Figure \ref{head}, where feature selection is conditional by applying instance-aware feature masks.

\subsection{Query Synthesis Module}
From the disentangled view of memory-efficient tuning, the model adapts to downstream tasks by training a task-specific learning module. Therefore, we propose a lightweight, trainable transformer block, named the Query Synthesis Module (QSM). This module is designed to capture task-specific features and synthesize them into task-specific queries for knowledge mining.

Specifically, when generating query tokens, we incorporate trainable random-initialized prompts at each layer in order to enable the model to fully capture task-specific features. Additionally, we observes that the results of previous queries are beneficial for the query in the subsequent block, indicating that knowledge mining should depend on previous results rather than being independent at each layer. Therefore, we integrate information from the previous layer's query results by adding them with the query prompt and finally generate synthesized query tokens. 

In Query Synthesis, the tokens interact with each other through attention layers, and are further fed into the feed-forward network for adaptation to the space of the ViT intermediate features $X_i$.  
Formally, given hidden size $d$, the query results from the last layer ${H}_{i}$ are added with trainable prompt $P_i$ and then fed into projection with bottleneck $r$ to obtain input of the attention layer $Z_i$.
\begin{equation}
    {F}_i^{qs} = (({H}_{i} + P_i)\mathbf{W}_{down})\mathbf{W}_{up},
\end{equation}
where projection is decomposed into $\mathbf{W}_{down}^{\cdot}\in \mathbb{R}^{d,r}$ and $\mathbf{W}_{up}^{\cdot}\in \mathbb{R}^{r,d}$.

In the attention layer, these query tokens are projected with another bottleneck module to obtain the query, key and value as follows. 

\begin{equation}
    \left\{
    \begin{aligned}
        Q^{qs}_i=f(\text{Norm}({Z}_i^{qs})\mathbf{W}_{down}^q)\mathbf{W}_{up}^q \\
        K^{qs}_i=f(\text{Norm}({Z}_i^{qs})\mathbf{W}_{down}^k)\mathbf{W}_{up}^k \\
        V^{qs}_i=f(\text{Norm}({Z}_i^{qs})\mathbf{W}_{down}^v)\mathbf{W}_{up}^v \\
    \end{aligned}
    \right.
    ,
\end{equation}
where $\text{Norm}(\cdot)$ represents normalization and $f(\cdot)$ denotes a nonlinear activation function. 
The hidden embedding after attention layers $\hat{F}_i^{qs}$ can be calculated as follows:  
\begin{equation}
    \hat{F}_i^{qs} = \text{Attn}(Q^{qs}_i, K^{qs}_i, V^{qs}_i) + {F}_i^{qs}.
\end{equation}
Then we can further obtain the hidden embedding after FFN layers as the input of Knowledge Extraction Module ${F}_i^{ke}$:
\begin{equation}
    {F}_i^{ke} = \text{FFN}(\text{Norm}(\hat{F}_i^{qs})) + \hat{F}_i^{qs}.
\end{equation}


\subsection{Knowledge Extraction Module}
With the task-specific synthesized query obtained from QSM, we can apply information mining by adopting Knowledge Extraction Module (KEM). Specifically, we take the synthesized query as the query in the KSM, and intermediate features  in the pre-trained model as key and value. To optimize parameter usage, all the parameters are inherited from the pre-trained ViT block and frozen during training. Formally, given task-specific synthesized query ${F}_i^{ke}$, normalization $\text{Norm}(\cdot)$ and projection layer $\mathbf{W}^q, \mathbf{W}^k, \mathbf{W}^v$ in the pre-trained ViT block, we obtain the query, key, value and hidden embedding after attention layers $\hat{F}_i^{ke}$ as follows:
\begin{equation}
    \left\{
    \begin{aligned}
        Q^{ke}_i=f(\text{Norm}({F}_i^{ke}))\mathbf{W}^q \\
        K^{ke}_i=f(\text{Norm}(X_{i}))\mathbf{W}^k             \\
        V^{ke}_i=f(\text{Norm}(X_{i}))\mathbf{W}^v             \\
    \end{aligned}
    \right.
    .
\end{equation}

\begin{equation}
    \hat{F}_i^{ke} = \text{Attn}(Q^{ke}_i, K^{ke}_i, V^{ke}_i) + {F}_i^{ke} .
\end{equation}
We also reuse the weight in the feed-forward network to perform the same space transformation as in the pretrained block: 
\begin{equation}
    {H}_i = \text{FFN}(\text{Norm}(\hat{F}_i^{ke})) + \hat{F}_i^{ke} .
\end{equation}
We observes that for the original ViT model, the classification task relies not only on the meaningful information contained within the query results, but also on the rich hierarchical features extracted during the knowledge mining. Thus, we additionally extract information after the Attention module and the Feed-Forward Network module, apart from the query results, for the final classification. These are denoted as $Z_i^{att}$ and $Z_i^{ffn}$, respectively:

\begin{equation}
    Z_i^{att} = \text{Attn}(Q^{ke}_i, K^{ke}_i, V^{ke}_i),
\end{equation}


\begin{equation}
    Z_i^{ffn} = \text{FFN}(\text{Norm}(\hat{F}_i^{ke})).
\end{equation}
The task-specific synthesized query results ${H}_i$, along with the rich hierarchical features $Z_i^{att}$ and $Z_i^{ffn}$, serve as beneficial information extracted from the entire intermediate features of the pre-trained ViT model for downstream tasks. We refer to all the features obtained from KSM, which are subsequently used as input to the final classification head, as mining features.


\subsection{Classification Head}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{pdf/head.pdf}
    \caption{Classification head for aggregating features.}
    \label{head}
\end{figure}
After information mining in the KSM, we obtain the query results of each layer along with the corresponding intermediate attention features $Z_i^{att}$ and FFN features $Z_i^{ffn}$. These features are rich and hierarchical, containing a large amount of information but also some redundancy. Therefore, it is crucial to perform feature selection, aiming to extract the truly beneficial information for downstream tasks.

Moreover, we observe a significant disparity in the data distribution across different downstream datasets, and there may be significant differences between samples as well. Motivated by this observation, we propose an instance-aware classification head and adaptively aggregate the features conditional on the final query results ${H}_n$ of the input sample, by generating a mask for all features to perform feature selection through mining.
Specifically, we project ${H}_n$ to obtain a mask for other mining features (excluding $\hat{H}_n$ itself). Then, we apply a projection with bottleneck to all mining features and apply weight sum to aggregate the projected features. Specifically, we set the mask weight of $\hat{H}_n$ to 1 during aggregation. The aggregated results are then fed into a Multi-Layer Perceptron (MLP) for classification.

Additionally, to enhance the model's robustness and prevent overfitting, we introduce DropPath into the input of other mining features, excluding the conditional token $\hat{H}_n$. This ensures that the model does not overly rely on a specific feature during training, which significantly improves the model's performance.

In the classification head, all projections are implemented using an adapter-like bottleneck module, which meets the requirement for a limited number of parameters. The result of the last layer query of the sample, $\hat{H}_n$, serves a role similar to the cls token in trainditional ViT. Our model generates a mask for other mining features based on it, making the classification head instance-aware.



\newpage

==> sec/main_result.tex <==
\begin{table*}[h]
    \vspace{-0.1in}
    \centering
    \caption{\textbf{Full results on VTAB-1K benchmark}. ``\# params'' specifies the number of trainable parameters {in backbones}. Average accuracy and \# params are averaged over group-wise mean values.}
    \label{tab:vtab}
    \setlength{\tabcolsep}{0.3pt}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{p{2.2cm}<{}p{0.9cm}<{\centering}|p{0.75cm}<{\centering}p{0.75cm}<{\centering}p{0.75cm}<{\centering}p{0.75cm}<{\centering}p{0.75cm}<{\centering}p{0.75cm}<{\centering}p{0.75cm}<{\centering}p{0.75cm}<{\centering}|p{0.75cm}<{\centering}p{0.75cm}<{\centering}p{0.75cm}<{\centering}p{0.75cm}<{\centering}|p{0.75cm}<{\centering}p{0.75cm}<{\centering}p{0.75cm}<{\centering}p{0.75cm}<{\centering}p{0.75cm}<{\centering}p{0.75cm}<{\centering}p{0.75cm}<{\centering}p{0.75cm}<{\centering}|p{0.75cm}<{\centering}}
            \toprule[1.5pt]
            \multicolumn{3}{c|}{}             & \multicolumn{7}{c|}{\textbf{Natural}}                           & \multicolumn{4}{c|}{\textbf{Specialized}} & \multicolumn{8}{c|}{\textbf{Structured}} &                                                                                                                                                      \\
                                              & \multicolumn{1}{c|}{{\rotatebox[origin=c]{90}{\# param (M)}}}
                                              & \multicolumn{1}{c|}{{\rotatebox[origin=c]{90}{Inference Cost}}}
                                              & \multicolumn{1}{c}{{\rotatebox[origin=c]{90}{Cifar100}}}
                                              & \multicolumn{1}{c}{{\rotatebox[origin=c]{90}{Caltech101}}}
                                              & \multicolumn{1}{c}{{\rotatebox[origin=c]{90}{DTD}}}
                                              & \multicolumn{1}{c}{{\rotatebox[origin=c]{90}{Flower102}}}
                                              & \multicolumn{1}{c}{{\rotatebox[origin=c]{90}{Pets}}}
                                              & \multicolumn{1}{c}{{\rotatebox[origin=c]{90}{SVHN}}}
                                              & \multicolumn{1}{c|}{{\rotatebox[origin=c]{90}{Sun397}}}
                                              & \multicolumn{1}{c}{{\rotatebox[origin=c]{90}{Camelyon}}}
                                              & \multicolumn{1}{c}{{\rotatebox[origin=c]{90}{EuroSAT}}}
                                              & \multicolumn{1}{c}{{\rotatebox[origin=c]{90}{Resisc45}}}
                                              & \multicolumn{1}{c|}{{\rotatebox[origin=c]{90}{Retinopathy}}}
                                              & \multicolumn{1}{c}{{\rotatebox[origin=c]{90}{Clevr-Count}}}
                                              & \multicolumn{1}{c}{{\rotatebox[origin=c]{90}{Clevr-Dist}}}
                                              & \multicolumn{1}{c}{{\rotatebox[origin=c]{90}{DMLab}}}
                                              & \multicolumn{1}{c}{{\rotatebox[origin=c]{90}{KITTI-Dist}}}
                                              & \multicolumn{1}{c}{{\rotatebox[origin=c]{90}{dSpr-Loc}}}
                                              & \multicolumn{1}{c}{{\rotatebox[origin=c]{90}{dSpr-Ori}}}
                                              & \multicolumn{1}{c}{{\rotatebox[origin=c]{90}{sNORB-Azim}}}
                                              & \multicolumn{1}{c|}{{\rotatebox[origin=c]{90}{sNORB-Ele}}}
                                              & \multicolumn{1}{c}{{\rotatebox[origin=c]{90}{Average}}}                                                                                                                                                                                                                                                       \\
            \specialrule{0em}{1pt}{1pt}
            \hline
            \specialrule{0em}{1pt}{1pt}
            \multicolumn{23}{l}{\emph{Traditional Finetuning}}                                                                                                                                                                                                                                                                                                \\
            \hline
            \specialrule{0em}{1pt}{1pt}
            Full                              & 85.8                                                            & -                                         & 68.9                                     & 87.7 & 64.3 & 97.2 & 86.9 & 87.4 & 38.8 & 79.7 & 95.7 & 84.2 & 73.9          & 56.3 & 58.6          & 41.7 & 65.5 & 57.5 & 46.7 & 25.7 & 29.1 & 68.9 \\
            Linear                            & 0                                                               & -                                         & 64.4                                     & 85.0 & 63.2 & 97.0 & 86.3 & 36.6 & 51.0 & 78.5 & 87.5 & 68.5 & 74.0          & 34.3 & 30.6          & 33.2 & 55.4 & 12.5 & 20.0 & 9.6  & 19.2 & 57.6 \\
            %\specialrule{0em}{1pt}{1pt}
            \hline
            \specialrule{0em}{1pt}{1pt}
            \multicolumn{23}{l}{\emph{PEFT methods}}                                                                                                                                                                                                                                                                                                          \\
            \hline
            \specialrule{0em}{1pt}{1pt}
            BitFit                            & 0.10                                                            & -                                         & 72.8                                     & 87.0 & 59.2 & 97.5 & 85.3 & 59.9 & 51.4 & 78.7 & 91.6 & 72.9 & 69.8          & 61.5 & 55.6          & 32.4 & 55.9 & 66.6 & 40.0 & 15.7 & 25.1 & 65.2 \\
            VPT-Shallow                       & 0.06                                                            & $\uparrow$                                & 77.7                                     & 86.9 & 62.6 & 97.5 & 87.3 & 74.5 & 51.2 & 78.2 & 92.0 & 75.6 & 72.9          & 50.5 & 58.6          & 40.5 & 67.1 & 68.7 & 36.1 & 20.2 & 34.1 & 67.8 \\
            VPT-Deep                          & 0.53                                                            & $\uparrow$                                & \textbf{78.8}                            & 90.8 & 65.8 & 98.0 & 88.3 & 78.1 & 49.6 & 81.8 & 96.1 & 83.4 & 68.4          & 68.5 & 60.0          & 46.5 & 72.8 & 73.6 & 47.9 & 32.9 & 37.8 & 72.0 \\
            Adapter                           & 0.16                                                            & $\uparrow$                                & 69.2                                     & 90.1 & 68.0 & 98.8 & 89.9 & 82.8 & 54.3 & 84.0 & 94.9 & 81.9 & 75.5          & 80.9 & 65.3          & 48.6 & 78.3 & 74.8 & 48.5 & 29.9 & 41.6 & 73.9 \\
            AdaptFormer                       & 0.16                                                            & $\uparrow$                                & 70.8                                     & 91.2 & 70.5 & 99.1 & 90.9 & 86.6 & 54.8 & 83.0 & 95.8 & 84.4 & \textbf{76.3} & 81.9 & 64.3          & 49.3 & 80.3 & 76.3 & 45.7 & 31.7 & 41.1 & 74.7 \\
            LoRA                              & 0.29                                                            & -                                         & 67.1                                     & 91.4 & 69.4 & 98.8 & 90.4 & 85.3 & 54.0 & 84.9 & 95.3 & 84.4 & 73.6          & 82.9 & \textbf{69.2} & 49.8 & 78.5 & 75.7 & 47.1 & 31.0 & 44.0 & 74.5 \\
            % NOAH &0.36&$\uparrow$&69.6&92.7&70.2&99.1&90.4&86.1&53.7&84.4&95.4&83.9&75.8&82.8&68.9&49.9&81.7&81.8&48.3&32.8&\textbf{44.2}&75.5\\
            % FacT &0.07&-&70.6&90.6&70.8&99.1&90.7&88.6&54.1&84.8&96.2&84.5&75.7&82.6&68.2&49.8&80.7&80.8&47.4&33.2&43.0&75.6\\
            % SSF &0.24&-& 69.0& 92.6& 75.1& 99.4& 91.8& 90.2& 52.9& 87.4& 95.9& 87.4& 75.5& 75.9& 62.3& 53.3& 80.6& 77.3& \textbf{54.9}& 29.5& 37.9&75.7\\
            % RepAdapter &0.22&-&72.4&91.6&71.0&99.2&91.4&90.7&55.1&85.3&95.9&84.6&75.9&82.3&68.0&50.4&79.9&80.4&49.2&38.6&41.0&76.1\\
            \hline
            \specialrule{0em}{1pt}{1pt}
            % \rowcolor{lightgray!30}\textbf{GLoRA}&0.86&-&76.4&\textbf{92.9}&74.6&99.6&\textbf{92.5}&\textbf{91.5}&\textbf{57.8}&87.3&\textbf{96.8}&88.0&76.0&\textbf{83.1}&67.3&\textbf{54.5}&\textbf{86.2}&\textbf{83.8}&52.9&\textbf{37.0}&41.4&\textbf{78.0}\\
            % \rowcolor{lightgray!30}\textbf{GLoRA}&0.44&-&76.5&92.3&75.2&99.6&92.3&91.2&57.5&87.3&96.7&88.1&76.1&80.6&67.2&53.4&84.5&83.5&52.8&35.2&40.8&77.6\\
            % \rowcolor{lightgray!30}\textbf{GLoRA}&0.29&-&76.1&92.7&\textbf{75.3}&\textbf{99.6}&92.4&90.5&57.2&\textbf{87.5}&96.7&\textbf{88.1}&76.1&81.0&66.2&52.4&84.9&81.8&53.3&33.3&39.8&77.3\\
            \rowcolor{lightgray}\textbf{Ours} &                                                                 & -                                         & 70.9
                                              & 89.7                                                            &
            68.8                              &
            98.5                              &
            89.6                              &
            77.8                              &
            50.6                              &
            82.3                              &
            96.7                              &
            83.5                              &
            75.2                              &
            71.8                              &
            62.7                              &
            48.5                              &
            75.4                              &
            74.1                              &
            49.0                              &
            31.7                              &
            36.1                              & 72.9                                                                                                                                                                                                                                                                                                          \\
            \bottomrule[1.5pt]
        \end{tabular}
    }
    \vspace{-0.06in}
\end{table*}
